Reducing Load Latency with Cache Level Prediction

High load latency that results from deep cache hierarchies and relatively slow main memory is an important limiter of single-thread performance. Data prefetch helps reduce this latency by fetching data up the hierarchy before it is requested by load instructions. However, data prefetching has shown to be imperfect in many situations. We propose cache-level prediction to complement prefetchers. Our method predicts which memory hierarchy level a load will access allowing the memory loads to start earlier, and thereby saves many cycles. The predictor provides high prediction accuracy at the cost of just one cycle added latency to L1 misses. Experimental results show speedup of 7.8\% on generic, graph, and HPC applications over a baseline with aggressive prefetchers.

==> background.tex <==
\section{Background}
\label{sec:background}
Modern processors employ three or more levels of cache. The cache levels are accessed in sequence. The first level cache (L1, the highest level cache) is looked up first, and in the case of a miss the request is forwarded to L2, and then L3 (the lowest level cache). If the data is not found in any cache, it is read from main memory. To provide non-blocking access, each cache has miss status holding registers (MSHRs). MSHRs track outstanding misses, allowing the processor to continue execution while a request is serviced. MSHRs also  coalesce different targets to the same cache block.  

% Multi-level cache hierarchies can be: (1) inclusive: all blocks present in a cache level must also be present in the lower level cache; (2) exclusive: blocks present in a cache level must not be present in a higher level cache; and (3) non-inclusive: blocks present in a cache may or may not be present in lower level caches.

%--------------------------------------------
% \begin{figure}[t]
% \centering
% \includegraphics[width=3in]{back.pdf}
  % \caption{An example of 3-level Cache hierarchy.}
% \label{fig:back}
% \end{figure}
%--------------------------------------------


% Recent Intel processors use a non-inclusive hierarchy \cite{InteSpec}. A typical cache hierarchy is shown in Figure \ref{fig:back} where L1 and L2 are inclusive while L2 and L3 are non-inclusive. First, we describe the operations on a fill in the inclusive part (L1+L2), and then explain the non-inclusive part (L3+L2).


% When L3 responds to a miss \ballnumber{1}, the L2 MSHR is checked and the block is filled. At the same time, the response is also sent to L1 \ballnumber{2}. In L1, we need to evict another block. Hence, a candidate is identified by the replacement policy and is then evicted \ballnumber{3}. The eviction causes a writeback to L2 if the block is dirty. When the block is evicted to L2, another block from L2 must be evicted to service this write-back \ballnumber{4}. Here is where the inclusion properties are enforced. A back invalidation request is sent to L1 to evict the L1 victim \ballnumber{6}. This back invalidation is necessary in inclusive caches as is the case for L1 and L2. In this example, invalidation guarantees that there would be no copy of the block in L1 while the block has been evicted from L2.

% For non-inclusive caches (L2+L3), when a request is responded, the back invalidation is not sent out to L2. Hence, L2 can hold a block, even when it is no longer present in L3.

% Mattan cut this too.
%Maintaining cache coherence in modern exclusive and non-inclusive cache hierarchies can be challenging. For example, when core 0 requests a block which is not present in L3, but is present in the L2 cache of core 1, we need a mechanism to redirect the request to L2 of core 1, and not to main memory. To address this issue, a directory structure is used. The directory keeps track of the latest location of any block in the chip, and thus redirects requests to the correct location. 

% The structure of the directory in recent Intel processors is discussed in \cite{Skylakedirectory} and shown in Figure \ref{fig:back}. 

%\subsection{Cache coherence directory}
% The directory is sliced and has the same number of sets as the LLC. An LLC slice can be collocated with its directory, enabling concurrent LLC slice and directory lookup \cite{Skylakedirectory}. The directory has 3 types of ways: (1) traditional ways, (2) extended ways, and (3) shared ways. The traditional ways hold the coherence information that is required in a traditional inclusive hierarchy: the L3 tags and the per-core coherence information. The extended ways hold additional coherence information for supporting non-inclusive hierarchies -- they store the address tags of the per-core L2 caches and allow L3 to act as a snoop filter. The shared ways are divided between traditional and extended ways at run-time by the replacement policy \cite{Skylakedirectory}. 

\madd{Current processors use a distributed directory to maintain coherence. The directory tracks the locations of any block in all on-chip caches to redirect requests and force write-backs and invalidations when necessary.}
% The directory can precisely locate a block present in any of the L2 caches or LLC. In a multi-core setting, when a request arrives at L3 for a block that is present in a lower level cache, the directory lookup is used to fetch data from the appropriate L2. This ensures that stale data is never returned by L3.
The directory plays a significant role in our design and we rely on it to resolve level mispredictions. Note that directory lookup does not replace cache level prediction. First it is located in or near the LLC tags, and thus far from the L2 cache. Second, the cost of the directory lookup is high and thus not beneficial from both latency and energy perspectives.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

